DDoD: Dual Denial of Decision Attacks on Human-AI Teams

Artificial Intelligence (AI) systems have been increasingly used to make decision-making processes faster, more accurate, and more efficient. However, such systems are also at constant risk of being attacked. While the majority of attacks targeting AI-based applications aim to manipulate classifiers or training data and alter the output of an AI model, recently proposed Sponge Attacks against AI models aim to impede the classifier's execution by consuming substantial resources. In this work, we propose \textit{Dual Denial of Decision (DDoD) attacks against collaborative Human-AI teams}. We discuss how such attacks aim to deplete \textit{both computational and human} resources, and significantly impair decision-making capabilities. We describe DDoD on human and computational resources and present potential risk scenarios in a series of exemplary domains.

==> cfp.tex <==

Title and abstracts due: 18 March 2022 (email to pvc1-2023@computer.org) \\
Full Manuscripts due: 1 April 2021 (via submission site) Publication: January-March 2023 \\

Call for Papers: Special Issue on Human-Centered AI Claudio Pinhanez, Florian Michahelles, Albrecht Schmidt Title and abstracts due: 18 March 2022 (email to pvc1-2023@computer.org) Full manuscripts due: 1 April 2022 (via submission site) Publication: January-March 2023 AI systems are being created that drive cars, determine where and which news and information people see, and make health decisions at home. These AI systems are increasingly used in devices and systems that are part of the pervasive computing fabric of the world, such as enabling physical games and supporting home and outdoor activities. A common thread of all these systems is the human element; people are critical in the design, operation, and use of those AI systems, and society has to ensure those systems operate transparently, promote equitable outcomes, respect privacy, and effectively serve people’s needs. AI systems are arguably at an adoption stage where it is easier to improve them by enhancing human interaction than by tinkering with architectures and models for gains in accuracy. This special issue of IEEE Pervasive Computing will have a focus on human-centered AI, providing a forum for papers investigating new forms of human-AI interactions and experiences that enhance and extend human capabilities in the context of pervasive applications and systems. We invite original and high-quality submissions addressing: - Theoretical and methodology papers focused on the intersection of human-centered AI and pervasive computing. - Exploration of novel user interfaces and modalities enabling seamless interaction between user and AI, such as in games, cars, and mobile apps. - Interaction metaphors and user interface concepts that enable joint control and demonstrate effective human-AI cooperation. - Methods and algorithms enabling human-AI collaboration and supporting users in better understanding decisions of AI-driven pervasive applications. - Seamless hand-over of control between user and AI, and vice versa. - Empowerment of users of pervasive systems to re-configure/re-train based on their experiences. - Evaluation of case studies of AI against human + AI. - Cases studies and lessons learned from experiments or large-scale rollout of human AI, such as in education, health, housing, transportation, work, and entertainment. - Human-centered security and privacy issues in AI deployments. Submissions tackling any aspect of this field are welcomed, as long as the connection to pervasive computing is clear and central to the paper. Review or summary articles—for example, critical evaluations of the state of the art, or an insightful analysis of established and upcoming technologies—may be accepted if they demonstrate academic rigor and relevance. Submission Guidelines For author information and guidelines on submission criteria, please visit the Author Information page. Please submit papers through the ScholarOne system, and be sure to select the special-issue name. Manuscripts should not be published or currently submitted for publication elsewhere. Please submit only full papers intended for review, not abstracts, to the ScholarOne portal. Abstracts should be sent by email to the guest editors directly. Guest Editors Contact the guest editors at pvc1-2023@computer.org. Claudio Pinhanez (IBM Research, Brazil) Florian Michahelles (TU Vienna, Austria) Albrecht Schmidt (LMU Munich, Germany)


Articles submitted to IEEE Pervasive Computing should not exceed 6,000 words, including all text, the abstract, keywords, bibliography, biographies, and table text. The word count should include 250 words for each table and figure. An article should have no more than 20 references (40 for survey papers). The abstract should be no more than 150 words and should describe the overall focus of your manuscript.



==> sections/7_references.tex <==
\begin{thebibliography}{1}




%
%\bibitem{AA1}
%O. Amft, J. Favela, S. Intille, M. Musolesi, and V. Kostakos, “Personalized Pervasive Health,” IEEE Pervasive Computing, vol. 19, pp. 11-13, 2020. (journal)
%
%\bibitem{BB1}
%M. Csikszentmihalyi, {\it Flow and the Foundations of Positive Psychology}, Springer, Dordrecht, 2014. (book)
%
%\bibitem{CC1}
%R. Larson, and M. Csikszentmihalyi, “The Experience Sampling Method,” Flow and the Foundations of Positive Psychology, Springer, Dordrecht, 2014. (book article)
%
%\bibitem{DD1}
%L. F. Barrett, R. Adolphs, S. Marsella, A. M. Martinez, and S. D. Pollak “Emotional Expressions Reconsidered: Challenges to Inferring Emotion From Human Facial Movements,” Psychological Science in the Public Interest, vol. 20, no. 1, pp. 1-68, 2019. (journal)
%
%\bibitem{EE1}
%A. Adams, and A. L. Cox, “Questionnaires, in-depth interviews and focus groups,” Research Methods for Human-Computer Interaction, Cambridge University Press, 2014. (book article)
%
%\bibitem{FF1}
%N. Bolger, A. Davis, and E. Rafaeli “Diary Methods: Capturing Life as it is Lived,” Annual Review of Psychology, vol. 54, pp. 579-616, 2003. (journal)
%
%\bibitem{GG1}
%N. van Berkel et al., “Effect of experience sampling schedules on response rate and recall accuracy of objective self-reports,” International Journal of Human Computer Studies., vol. 125, pp. 118-128, 2019. (journal)
%
%\bibitem{HH1}
%Z. Sarsenbayeva et al., “Does Smartphone Use Drive our Emotions or vice versa? A Causal Analysis,” 2020 ACM Int. Conference on Human Factors in Computing Systems, 2020. (conference proceedings)
%
%\bibitem{II1}
%Z. Sarsenbayeva, B. Tag, S. Yan, V. Kostakos, and J. Goncalves, “Using Video Games to Regulate Emotions,” 32nd Australian Conference on Human-Computer Interaction, pp. 755-759, 2020. (conference proceedings)
%
%
%\bibitem{JJ1}
%J. Goncalves et al., “Projective testing of diurnal collective emotion,” Proceedings of the 2014 ACM International Joint Conference on Pervasive and Ubiquitous Computing, pp. 487-497, 2014. (conference proceedings)
%
%
%\bibitem{KK1}
%T. Dingler, B. Tag, S. Lehrer, and A. Schmidt, “Reading Scheduler: Proactive Recommendations to Help Users Cope with Their Daily Reading Volume,” Proceedings of the 17th International Conference on Mobile and Ubiquitous Multimedia, pp. 239-244, 2018. (conference proceedings)
%
%\bibitem{LL1}
%B. Tag, A. W. Vargo, A. Gupta, G. Chernyshov, K. Kunze, and T. Dingler, “Continuous Alertness Assessments: Using EOG Glasses to Unobtrusively Monitor Fatigue Levels In-The-Wild,” in Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems, 2019, pp. 464:1--464:12. (conference proceedings)
%
%\bibitem{MM1}
%S. Weller, “Using internet video calls in qualitative (longitudinal) interviews: some implications for rapport,” International Journal of Social Research Methodology, vol. 20, no. 6, pp. 613-625, 2017. (journal)
%
%
%\bibitem{NN1}
%J. Sun, M. Rhemtulla, and S. Vazire, “Eavesdropping on Missing Data: What Are University Students Doing When They Miss Experience Sampling Reports?,” Personality and Social Psychology Bulletin, 2020. (journal)
%
%
%\bibitem{OO1}
%E. K. Kalokerinos et al., “Neuroticism may not reflect emotional variability,” Proceedings of the National Academy of Sciences of the United States of America, vol. 117, no. 17, pp. 9270-9276, 2020. (journal)
%
%
%\bibitem{PP1}
%P. Verduyn, and S. Lavrijsen, “Which emotions last longest and why: The role of event importance and rumination,” Motivation and Emotion, vol. 39, no. 1, pp. 119–127, 2015. (journal)
%
%
%\bibitem{QQ1}
%A. Dzedzickis, A. Kaklauskas, and V. Bucinskas, “Human emotion recognition: Review of sensors and methods,” Sensors (Switzerland), vol. 20, no. 3, 2020. (journal)
%
%
%\bibitem{RR1}
%K. Yang et al., “Benchmarking commercial emotion detection systems using realistic distortions of facial image datasets,” The Visual Computer, pp. 1–20, 2020. (journal)
%
%
%\bibitem{SS1}
%K. Caine, “Local Standards for Sample Size at CHI,” Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems, pp. 981–992, 2016. (conference proceedings)
%
%
%\bibitem{TT1}
%P. Klasnja et al., “Microrandomized trials: An experimental design for developing just-in-time adaptive interventions,” Health Psychology, vol. 34, no. S, 2015. (journal)


\end{thebibliography}
